Quantifying Program Bias

With the range and sensitivity of algorithmic decisions expanding at a break-neck speed, it is imperative that we aggressively investigate whether programs are biased. We propose a novel probabilistic program analysis technique and apply it to quantifying bias in decision-making programs. Specifically, we (i) present a sound and complete automated verification technique for proving quantitative properties of probabilistic programs; (ii) show that certain notions of bias, recently proposed in the fairness literature, can be phrased as quantitative correctness properties; and (iii) present FairSquare, the first verification tool for quantifying program bias, and evaluate it on a range of decision-making programs.

==> alg.tex <==
\section{Fairness-Verification Algorithm}\label{sec:alg}

\todo{Turn this into a case study.
Begin by introducing the notion of group fairness
similar to the current intro section.}

Now that we have fully introduced our volume-computation
technique, we are ready to present the fairness-verification algorithm.
Recall that in an $\epsilon$-fairness problem, $(\pre, \dec, \post)$,
we would like to prove or disprove the probabilistic postcondition $(\post)$:
$$\frac{\pr{\varphi_f \mid \varphi_s}}{
        \pr{\varphi_f \mid \neg \varphi_s}} > 1 - \epsilon$$
To prove this statement, we need to compute
a value for the numerator and the denominator. However,
recall that $\volalg$ maintains a \emph{lower bound} on the
probability. Therefore, we have to be careful in how we use its results.
Specifically, to prove fairness, we need a lower bound on
the numerator and an upper bound on the denominator---these bounds allow
us to compute a lower bound on the ratio.
Conversely, to prove unfairness, we require
an upper bound on the numerator
and a lower bound on the denominator.

First, let us rewrite $\post$ to get rid of conditional probabilities,
using the axiom $\pr{A \mid B} = \pr{A \land B} / \pr{B}$:
$$\frac{\pr{\varphi_f \land \varphi_s} \cdot \pr{\neg \varphi_s}}
{\pr{\varphi_f \land \neg \varphi_s} \cdot \pr{\varphi_s}}
> 1-\epsilon
$$
As in the abstract verification algorithm from Figure~\ref{alg:verify},
we have the probabilistic verification condition, $\pair{\varphi_\prog, \pdfs}$,
and the set of variables $V_d = V_d^\emph{pre} \cup V_d^\emph{dec}$.
To find a lower bound on the probability of some property $\varphi$,
denoted by $\prl{\varphi}$, we can invoke $\volalg(\exists V_d \ldotp \semprog \land \varphi, \pdfs)$.
Conversely, following Corollary~\ref{col:upper}, to find an upper bound $\pru{\varphi}$,
we can compute $1 - \volalg(\neg \exists V_d \ldotp \semprog \land \varphi, \pdfs).$

Our fairness algorithm is shown in Figure~\ref{alg:fairsquare}.
We assume that the function \textsc{updateProbabilities}
runs \volalg for a limited amount of iterations to
improve the upper and lower bounds on the various
properties, $\pr{\varphi_f \land \varphi_s}$, $\pr{\varphi_s}$, etc.
Thus, the algorithm simply loops, and in every iteration checks
whether we can prove fairness or unfairness.
Specifically, it first computes a lower bound
on the ratio
$\frac{\pr{\varphi_f \mid \varphi_s}}{
        \pr{\varphi_f \mid \neg \varphi_s}}$;
if the lower bound is greater than $1-\epsilon$,
then the problem is definitely fair.
The algorithm then proceeds to compute an upper
bound on the ratio, and if the upper bound is $\leq 1-\epsilon$,
we know that the problem is definitely unfair.

\paragraph{Soundness and completeness}
The following theorem states
soundness and (\emph{almost}) completeness
of \textsc{fairVerify}.
Completeness of the algorithm
is contingent on two factors.
First, \volalg should in the limit
converge to exact solutions.
If the problem is fair, then, in finitely many steps,
 we will be able to prove that the ratio is $> 1-\epsilon$.
However, in the rare chance that
the ratio $\frac{\pr{\varphi_f \mid \varphi_s}}{
        \pr{\varphi_f \mid \neg \varphi_s}}$
        is \emph{exactly}  $1 - \epsilon$,
we might not be able to prove that the algorithm
is unfair, as our upper bound on the ratio will come closer
and closer to $1 - \epsilon$, but potentially
never reach it.


\begin{theorem}[Correctness of \textsc{fairVerify}]\label{thm:fair}
Fix a fairness verification problem $(\pre, \dec, \post)$.
%
%\begin{itemize}
%
%\item
\textbf{Soundness}:
If \textsc{fairVerify} returns fair or unfair,
the result is correct.
%
%\item
\textbf{Almost completeness}:
If $\frac{\pr{\varphi_f \mid \varphi_s}}{
        \pr{\varphi_f \mid \neg \varphi_s}} \neq 1 - \epsilon$,
then \textsc{fairVerify} eventually
terminates.
%\end{itemize}
\end{theorem}

\begin{figure}[!t]
  \small
  \begin{spacing}{1}
    \begin{algorithmic}
        \Function{fairVerify}{$\pre, \dec, \post$}
          % \State Let $\varphi_\prog$ and $\pdfs$ be as in Figure~\ref{alg:verify}
          % \State Fork the following \volalg processes
          % \State $\prl{\varphi_f\land\varphi_s} \gets \volalg( \exists V_d \ldotp \varphi_\prog \land \varphi_s \land \varphi_f, \pdfs) $
          % \State $\pru{\varphi_f\land\varphi_s} \gets 1 - \volalg(\neg \exists V_d \ldotp \varphi_\prog \land \varphi_s \land \varphi_f, \pdfs) $
          % \State
          % \State $\prl{\varphi_f\land \neg \varphi_s} \gets \volalg( \exists V_d \ldotp \varphi_\prog \land \neg \varphi_s \land \varphi_f, \pdfs) $
          % \State $\pru{\varphi_f\land \neg\varphi_s} \gets 1 - \volalg(\neg \exists V_d \ldotp \varphi_\prog \land \neg \varphi_s \land \varphi_f, \pdfs) $
          % \State
          % \State $\prl{\varphi_s} \gets \volalg( \exists V_d \ldotp \varphi_\prog \land \varphi_s, \pdfs) $
          % \State $\pru{\varphi_s} \gets 1 - \volalg(\neg \exists V_d \ldotp \varphi_\prog \land \neg \varphi_s \land \varphi_f, \pdfs) $
          \While {$\true$}

			~~~~~~~\Call{updateProbabilities}{\hspace{0mm}}

            {\color{darkgray}{~~~~~~~// compute lower bound on ratio}}
            \begin{align*}
              \textbf{if}~~
            \frac{\prl{\varphi_f \land \varphi_s} \cdot \prl{\neg \varphi_s}}
            {\pru{\varphi_f \land \neg \varphi_s} \cdot \pru{\varphi_s}}
            > 1-\epsilon & &
          \end{align*}
               \hspace{.7in}\Return fair


               {\color{darkgray}{~~~~~~~// compute upper bound on ratio}}
              \begin{align*}
                \textbf{if}~~
              \frac{\pru{\varphi_f \land \varphi_s} \cdot \pru{\neg \varphi_s}}
              {\prl{\varphi_f \land \neg \varphi_s} \cdot \prl{\varphi_s}}
              \leq  1-\epsilon & &
            \end{align*}
                 \hspace{.7in}\Return unfair
            \EndWhile
        \EndFunction
    \end{algorithmic}
    \caption{Fairness verification algorithm}\label{alg:fairsquare}
  \end{spacing}
\end{figure}


==> bigtable.tex <==
\begin{table*}[]
\newcommand{\qentry}[9]{#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8 & #9}
\centering
\begin{tabular}{|c|c|c|c|c||cc||cc|cc|cc|}
\cline{2-13}
\multicolumn{1}{c|}{} & Dist Approx & Sample Max & Round & Time (s) & \multicolumn{2}{c||}{Fairness} & \multicolumn{2}{c|}{$\pr{\varphi_s}$} & \multicolumn{2}{c|}{$\pr{\varphi_f \land \varphi_s}$} & \multicolumn{2}{c|}{$\pr{\varphi_f \land \lnot \varphi_s}$} \\ \hline
\multirow{24}{*}{DT4} & \multirow{4}{*}{none} & \multirow{4}{*}{no} 
                     & 1 & \qentry{0.56}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-11}$}{1.00} \\
                 & & & 2 & \qentry{0.67}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-11}$}{0.99} \\ 
                 & & & 3 & \qentry{0.78}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-12}$}{0.99} \\ 
                 & & & 4 & \qentry{0.90}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-12}$}{0.99} \\ \cline{2-13}
                     & \multirow{4}{*}{uniform} & \multirow{4}{*}{no} 
                     & 1 & \qentry{0.41}{0.01}{40.32}{0.33}{0.33}{0.00}{0.33}{0.02}{0.67} \\
                 & & & 2 & \qentry{0.57}{0.06}{13.23}{0.33}{0.33}{0.01}{0.33}{0.05}{0.34} \\ 
                 & & & 3 & \qentry{0.72}{0.08}{12.69}{0.33}{0.33}{0.01}{0.32}{0.05}{0.34} \\ 
                 & & & 4 & \qentry{0.88}{0.08}{7.60}{0.33}{0.33}{0.01}{0.29}{0.08}{0.34} \\ \cline{2-13}
                     & \multirow{4}{*}{5 steps} & \multirow{4}{*}{no} 
                     & 1 & \qentry{0.70}{0.21}{7.50}{0.33}{0.33}{0.05}{0.35}{0.09}{0.50} \\
                 & & & 2 & \qentry{1.01}{0.27}{3.98}{0.33}{0.33}{0.06}{0.23}{0.12}{0.41} \\ 
                 & & & 3 & \qentry{1.37}{0.43}{2.56}{0.33}{0.33}{0.06}{0.16}{0.12}{0.27} \\ 
                 & & & 4 & \qentry{1.80}{0.45}{2.20}{0.33}{0.33}{0.06}{0.14}{0.13}{0.26} \\ \cline{2-13}
                     & \multirow{4}{*}{none} & \multirow{4}{*}{yes} 
                     & 1 & \qentry{0.73}{0.00}{11.20}{0.33}{1.00}{0.08}{1.00}{0.18}{0.58} \\
                 & & & 2 & \qentry{0.90}{0.62}{11.20}{0.33}{0.33}{0.08}{1.00}{0.18}{0.29} \\ 
                 & & & 3 & \qentry{1.04}{0.63}{8.86}{0.33}{0.33}{0.09}{0.79}{0.18}{0.29} \\ 
                 & & & 4 & \qentry{1.20}{0.63}{8.86}{0.33}{0.33}{0.09}{0.79}{0.18}{0.29} \\ \cline{2-13}
                     & \multirow{4}{*}{uniform} & \multirow{4}{*}{yes} 
                     & 1 & \qentry{0.70}{0.27}{3.71}{0.33}{0.33}{0.09}{0.33}{0.18}{0.67} \\
                 & & & 2 & \qentry{0.86}{0.54}{2.00}{0.33}{0.33}{0.09}{0.18}{0.18}{0.33} \\ 
                 & & & 3 & \qentry{1.04}{1.00}{1.00}{0.33}{0.33}{0.09}{0.09}{0.18}{0.18} \\ 
                 & & & 4 & \qentry{1.14}{1.00}{1.00}{0.33}{0.33}{0.09}{0.09}{0.18}{0.18} \\ \cline{2-13}
                     & \multirow{4}{*}{5 steps} & \multirow{4}{*}{yes} 
                     & 1 & \qentry{0.98}{0.26}{3.70}{0.33}{0.33}{0.08}{0.33}{0.18}{0.66} \\
                 & & & 2 & \qentry{1.17}{0.50}{2.00}{0.33}{0.33}{0.09}{0.18}{0.18}{0.36} \\ 
                 & & & 3 & \qentry{1.36}{1.00}{1.00}{0.33}{0.33}{0.09}{0.09}{0.18}{0.18} \\ 
                 & & & 4 & \qentry{1.47}{1.00}{1.00}{0.33}{0.33}{0.09}{0.09}{0.18}{0.18} \\ \hhline{|=|=|=|=|=#==#==|==|==|}
\multirow{24}{*}{SVM3} & \multirow{4}{*}{none} & \multirow{4}{*}{no} 
                      & 1 & \qentry{0.57}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-11}$}{1.00} \\
                  & & & 2 & \qentry{0.69}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-11}$}{1.00} \\ 
                  & & & 3 & \qentry{0.80}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-11}$}{1.00} \\ 
                  & & & 4 & \qentry{0.91}{0.00}{$10^{11}$}{0.33}{1.00}{$10^{-12}$}{1.00}{$10^{-11}$}{1.00} \\ \cline{2-13}
                      & \multirow{4}{*}{uniform} & \multirow{4}{*}{no} 
                      & 1 & \qentry{0.44}{0.02}{129.07}{0.25}{0.33}{0.01}{0.33}{0.01}{0.99} \\
                  & & & 2 & \qentry{0.65}{0.07}{19.46}{0.33}{0.33}{0.03}{0.33}{0.03}{0.98} \\ 
                  & & & 3 & \qentry{0.81}{0.11}{11.84}{0.33}{0.33}{0.04}{0.33}{0.06}{0.71} \\ 
                  & & & 4 & \qentry{0.99}{0.11}{11.01}{0.33}{0.33}{0.04}{0.32}{0.06}{0.70} \\ \cline{2-13}
                      & \multirow{4}{*}{5 steps} & \multirow{4}{*}{no} 
                      & 1 & \qentry{0.74}{0.09}{3.01}{0.25}{0.33}{0.03}{0.33}{0.33}{0.75} \\
                  & & & 2 & \qentry{1.31}{0.18}{1.15}{0.33}{0.33}{0.04}{0.19}{0.33}{0.42} \\ 
                  & & & 3 & \qentry{1.84}{0.27}{1.09}{0.33}{0.33}{0.06}{0.18}{0.33}{0.41} \\ 
                  & & & 4 & \qentry{2.45}{0.31}{1.08}{0.33}{0.33}{0.06}{0.18}{0.33}{0.39} \\ \cline{2-13}
                      & \multirow{4}{*}{none} & \multirow{4}{*}{yes} 
                      & 1 & \qentry{0.77}{0.00}{10.39}{0.33}{1.00}{0.10}{1.00}{0.19}{0.79} \\
                  & & & 2 & \qentry{1.10}{0.25}{8.21}{0.33}{0.33}{0.10}{0.79}{0.20}{0.79} \\ 
                  & & & 3 & \qentry{1.43}{0.25}{8.20}{0.33}{0.33}{0.10}{0.79}{0.20}{0.79} \\ 
                  & & & 4 & \qentry{1.83}{0.25}{8.19}{0.33}{0.33}{0.10}{0.79}{0.20}{0.79} \\ \cline{2-13}
                      & \multirow{4}{*}{uniform} & \multirow{4}{*}{yes} 
                      & 1 & \qentry{0.65}{0.34}{2.00}{0.33}{0.33}{0.17}{0.33}{0.33}{0.98} \\
                  & & & 2 & \qentry{1.03}{0.40}{1.00}{0.33}{0.33}{0.17}{0.17}{0.33}{0.83} \\ 
                  & & & 3 & \qentry{1.47}{0.49}{1.00}{0.33}{0.33}{0.17}{0.17}{0.33}{0.68} \\ 
                  & & & 4 & \qentry{1.99}{0.97}{1.00}{0.33}{0.33}{0.17}{0.17}{0.33}{0.34} \\ \cline{2-13}
                      & \multirow{4}{*}{5 steps} & \multirow{4}{*}{yes} 
                      & 1 & \qentry{0.94}{0.25}{2.00}{0.33}{0.33}{0.09}{0.33}{0.33}{0.75} \\
                  & & & 2 & \qentry{1.51}{0.89}{1.00}{0.33}{0.33}{0.17}{0.17}{0.33}{0.38} \\ 
                  & & & 3 & \qentry{2.38}{0.98}{1.00}{0.33}{0.33}{0.17}{0.17}{0.33}{0.34} \\ 
                  & & & 4 & \qentry{3.44}{0.99}{1.00}{0.33}{0.33}{0.17}{0.17}{0.33}{0.34} \\ \hline
\end{tabular}
\caption{A table illustrating how each of our various optimizations affect
the performance of \fs.  The population model used throughout is
the set of independent variables.  Each instance shows the intermediate calculations
for each of the first 4 rounds of volume computation.
The four leftmost columns show the lower and upper bounds for their
corresponding values.}
\label{tbl:opt}
\end{table*}




==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

We addressed the verification problem of group fairness
and implemented our tool, \fs, 
that utilizes a novel weighted volume computation algorithm 
to prove the fairness or unfairness of programs.
%
Our goals for future work include
exploring the applicability of our technique
to \emph{individual fairness}~\cite{dwork12};
further refinements to the use of \abrs{ADF},
e.g. dynamically adapting them during \volopt;
and improving the weighted volume computation algorithm
for better scalability in the number of variables.



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this section we discuss rationale behind the important design decisions that were made in this paper.

\todo{This paragraph is no longer very interesting}
We start by explaining why our new definition of group fairness uses a population model
instead of a concrete dataset.
Existing definitions of fairness define programs as fair or unfair with respect to a given concrete dataset, e.g.,~\cite{feldman15,dwork12}.
While using a concrete dataset simplifies the verification problem,
it also raises questions of whether
the dataset is representative for the population for which we are trying to prove fairness.
%Moreover, sensitive datasets are unlikely to be publicly available.
Our technique moves away from concrete datasets and replaces them with a  probabilistic population model.
Population models subsume concrete datasets and do not require making datasets publicly available.
Building a representative population model can be challenging; however, we envision a future in which
governmental agencies will publish representative population models and use them to assess
 fairness of algorithmic processes. The European Union (EU), for instance, has already begun regulating algorithmic decision-making~\cite{Goodman16}.

We presented an algorithm for exact volume computation (probabilistic inference) instead of using
existing techniques for approximate volume computation
or probabilistic inference, e.g. \emph{Metropolis--Hastings}~\cite{chib1995understanding} or
convex volume approximation~\cite{vempala2005geometric}.
Approximation techniques trade soundness for performance,
but soundness is fundamental for checking algorithm fairness:
%We can't conclude that an algorithm is more or less fair.
Our technique allows us to generate a checkable
\emph{certificate of fairness}, which is the set of sampled hyperrectangles.
Moreover, since our algorithm computes several individual quantities and then combines them,
inexact methods might end up accumulating error and producing very inaccurate results.

\todo{Need to rethink this justification}
While the technique we proposed is fairly general and captures many interesting machine-learning
classifiers, our goal is to build a fairness verifier and not a general-purpose
probabilistic program verifier.
For this reason, our language only contains constructs
that are used in classes of programs
where we might be interested in reasoning about fairness.
For instance, a majority of classifiers
synthesized by machine-learning algorithms are loop-free
programs that operate over real-valued inputs,
which our program model is able to capture.
% For example, our tool only allows distributions with constant parameters---e.g., mean and standard deviation.

%!TEX root = paper.tex

